Intelligent Decision Assistance Versus Automated Decision-Making: Enhancing Knowledge Work Through Explainable Artificial Intelligence

While recent advances in AI-based automated decision-making have shown many benefits for businesses and society, they also come at a cost. It has for long been known that a high level of automation of decisions can lead to various drawbacks, such as automation bias and deskilling. In particular, the deskilling of knowledge workers is a major issue, as they are the same people who should also train, challenge and evolve AI. To address this issue, we conceptualize a new class of DSS, namely Intelligent Decision Assistance (IDA) based on a literature review of two different research streams -- DSS and automation. IDA supports knowledge workers without influencing them through automated decision-making. Specifically, we propose to use techniques of Explainable AI (XAI) while withholding concrete AI recommendations. To test this conceptualization, we develop hypotheses on the impacts of IDA and provide first evidence for their validity based on empirical studies in the literature.

==> 0_ideas.tex <==
%"Third, these augmentations require neither perfect accuracy nor exhaustive modeling of the user’stasktobe useful (e.g., consider the subtask of “spelling” vs. the more general perfect accuracy nor exhaustive modeling of the user’stasktobe useful (e.g., consider the subtask of “spelling” vs. the more general goal of “writing”). " \cite{heer2019agency} level of decisions?


Intro

\citet{Parasuraman2000} defines ten different levels of automation, ranging from pure human decision-making to full automation. What all levels have in common is that after the initial human level they provide decision recommendations. The traditional school of information systems (IS) research, however, sees a sub-class before level two that does not provide decision recommendations, namely data-based decision support systems \cite{Power2008}.

%Todo: Add discussion about possible constructs like engagement

%TODO: Maybe map all to intelligent automation

%TODO: Maybe add here summary what we have learned from both research streams

%\textbf{Jurisdiction Decision Support Systems}:
%\cite{wadsworth2018achieving}

%\textbf{Public Sector Decision Support Systems}:
%\cite{mehdiyev2021explainable}

%\textbf{Recruiting Decision Support Systems}: 


%\Cref{tab:automation_levels} visualizes these 10 levels. 
%In general, we can differentiate between model-based and data-based DSSs. 
%History
%Below we briefly outline the history of DSSs. DSS history dates back to the late 1960s with studying computerized quantitative models to support decision making \cite{power2008decision}. The precursors of DSSs were Management Information Systems (MISs), which provide management with structured, periodic reports based on transactional data \cite{power2008decision}. The term DSS first appeared in \cite{gorry1971framework} \cite{arnott2005critical}. General theory development of DSSs begun in the mid to late 1970s \cite{power2007brief}. The earliest DSSs are personal decision support systems (PDSSs), which are small-scale information systems, developed for one or a small group of managers to support their decision-making \cite{arnott2012design}. From PDSSs three main research streams developed: Information systems to support group-based decision, systems based on artificial intelligence (AI) and data-driven DSSs. Group support systems (GSSs) were developed to support decision finding and making in groups  \cite{arnott2012design}. Based on the GSS, negotiation support systems (NSSs) developed, which support negotiation making. Intelligent decision support systems (IDSSs) incorporate methods from the artificial intelligence field. In 1981 the framework for knowledge-management based DSS (KMDSS) was developed \cite{power2007brief}. KMDSS support decision-making by providing functions for knowledge storage, retrieval, transfer, and application \cite{arnott2012design}.Regarding data-driven DSSs, in 1979 the foundation for executive information systems (EISs) was laid, which display critical success metrics for managers \cite{power2007brief}. Based on the EIS, data warehousing (DW) developed, which provides large-scale data infrastructure, by combing multiple databases to support decision makers with information \cite{arnott2012design}. From EIS and DW business intelligence (BI) developed. The term BI was mainly coined by Howard Dresner in 1989 \cite{power2007brief}.  BI and DSS differ in the following points: Most DSSs are built to directly support specific decision-making \cite[p. 24]{turban2010decision}. BI on the other side, supports decision-making indirectly by providing information \cite[p. 24]{turban2010decision}. Furthermore, BI is mostly supported by commercially available tools, whereas DSSs are specialized developed software \cite[p. 24]{turban2010decision}. From traditional BI, analytics evolved \cite{watson2014tutorial}. \cite{watson2014tutorial} discuss three different interpretations of the term analytics: First, it can be seen as an umbrella term for data analysis applications. The second interpretation is that analytics is the reporting part of BI. Lastly, analytics can be interpreted as the application of ``rocket science'' algorithms \cite[p. 1250]{watson2014tutorial}. Usually, the context makes clear which interpretation fits \cite{watson2014tutorial}. Analytics itself can be categorized into three fields, descriptive, predictive, and prescriptive analytics \cite{watson2014tutorial}. Descriptive analytics incorporates methods of traditional BI \cite{watson2014tutorial}. Predictive analytics refers to analyses about the future \cite{watson2014tutorial}. Additionally, it includes exploratory analytics \cite{watson2014tutorial}. Lastly, prescriptive analytics suggests actions \cite{watson2014tutorial}. 

%After discussing the history of DSSs in the following we will briefly present two key concepts of DSSs, namely the decision-making process and decisional guidance.


%\begin{table*}[thb]
%\centering
%\caption{\label{automation_levels} Levels of automation %\cite{Parasuraman2000} \vskip 3pt }
%\label{tab:automation_levels}
%\resizebox{\columnwidth*2}{!}{%
%\begin{tabular}{c|ll}
%\hline \bf Level & \bf Automation &  \\ \hline
%1 & The computer offers no assistance: human must take all decisions and actions  \\
%2 & The computer offers a complete set of decision/action alternatives, or %\\
%3 & narrows the selection down to a few, or \\
%4 & suggests one alternative, and   \\
%5 & executes that suggestion if the human approves, or…  \\
%6 & allows the human a restricted time to veto the suggestion before %automatic execution, or \\
%7 & executes automatically, then necessarily informs the human, and \\
%8 & informs the human only if asked or  \\ 
%9 & informs the human only if it, the computer, decides to  \\
%10 & The computer decides everything and acts autonomously, ignoring the %human.  \\
%\hline
%\end{tabular}}%
%\end{table*}

Conceptualisation
%Analogies
%This idea can be validated through the following three analogies: %TODO: add descriptions
%Children learning
%Children learn better by examples 
%Brainstorming
%Consultant analogy
%An other analogy would be the consulting business. A good consultant will never just tell you what to do but more inspire you and give insights.

%Discuss Morana framework

%The literature proposes taxonomies to determine appropriate LoA (e.g. Bainbridge 1983; Baxter et al. 2012; Chialastri 2012; Endsley and Kaber 1999; Kaber and Endsley 2004; Vagia et al. 2016) spanning from fully manual to full automation (Vagia et al. 2016).

%everything after data-based DSS we call automated decision making
%Suggestive guidance between 1 and 2

%\cite{russel2013artificial} discuss in their book that AI needs sensors and actuators. Following the four parts of automation, sensors would be a form of information acquisition automation and actuators a form of action automation. %add page

We propose a decision support system design that is enhanced by AI but does not display a particular AI recommendation and therefore would be positioned between data-based DSS and level two of \cite{Parasuraman2000} automation levels.

%further ideas
    %unsupervised ML
    %most experts are interested in diagnostics that come through XAI
    %Imperfect vs perfect systems
    %Bidirectional learning


Illustration
%\cite{wang2016deep} for example develop an AI (more specific a Deep Learning solution) to identify metastatic breast cancer. 
%As a first step, the researchers conduct an automatic information acquisition and they separate the breast from a white background. Finally they provide a probability map. The researchers



%"Even the most auto- mated systems, however, rely on experts and managers to maintain rules and monitor results." \cite{Harris2005}.

%XAI, expost

"Arnold and Sutton (1998) began work on the theory of technology dominance over concerns about the unintended consequences of the use of knowledge-based systems—decision-aiding technologies with embedded artificial intelligence (AI) components. Today, not only are these unintended consequences becoming increasingly clear, but
organizations’"

%TODO: Add table with summary
%\begin{table}[thb]
%\centering
%\caption{ Validation study results \vskip 3pt }
%\label{tab:validation_study}
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{c|ll}
%\hline \bf Source &\bf Performance   \\ \hline
%\cite{alqaraawi2020evaluating} &   \\
%\cite{carton2020feature} &  \\
%\cite{chu2020visual} &  \\
%\cite{lai2019human} &  \\
%\cite{lai2020chicago} & \\
%\cite{schmidt2019quantifying} &  \\
%\hline
%\end{tabular}}%
%\end{table}


==> 6.1_Preliminary_design.tex <==
%Design elements
%Interactivity Shneiderman
%"These aids blend into the interactive experience in a non disruptive manner and can be directly invoked or dismissed."\cite{heer2019agency}

